Do-Operation Guided Causal Representation Learning with Reduced Supervision Strength

Causal representation learning has been proposed to encode relationships between factors presented in the high dimensional data. However, existing methods suffer from merely using a large amount of labeled data and ignore the fact that samples generated by the same causal mechanism follow the same causal relationships. In this paper, we seek to explore such information by leveraging do-operation to reduce supervision strength. We propose a framework that implements do-operation by swapping latent cause and effect factors encoded from a pair of inputs. Moreover, we also identify the inadequacy of existing causal representation metrics empirically and theoretically and introduce new metrics for better evaluation. Experiments conducted on both synthetic and real datasets demonstrate the superiorities of our method compared with state-of-the-art methods.

==> math_commands.tex <==
%%%%% NEW MATH DEFINITIONS %%%%%

\usepackage{amsmath,amsfonts,bm}

% Mark sections of captions for referring to divisions of figures
\newcommand{\figleft}{{\em (Left)}}
\newcommand{\figcenter}{{\em (Center)}}
\newcommand{\figright}{{\em (Right)}}
\newcommand{\figtop}{{\em (Top)}}
\newcommand{\figbottom}{{\em (Bottom)}}
\newcommand{\captiona}{{\em (a)}}
\newcommand{\captionb}{{\em (b)}}
\newcommand{\captionc}{{\em (c)}}
\newcommand{\captiond}{{\em (d)}}

% Highlight a newly defined term
\newcommand{\newterm}[1]{{\bf #1}}


% Figure reference, lower-case.
\def\figref#1{figure~\ref{#1}}
% Figure reference, capital. For start of sentence
\def\Figref#1{Figure~\ref{#1}}
\def\twofigref#1#2{figures \ref{#1} and \ref{#2}}
\def\quadfigref#1#2#3#4{figures \ref{#1}, \ref{#2}, \ref{#3} and \ref{#4}}
% Section reference, lower-case.
\def\secref#1{section~\ref{#1}}
% Section reference, capital.
\def\Secref#1{Section~\ref{#1}}
% Reference to two sections.
\def\twosecrefs#1#2{sections \ref{#1} and \ref{#2}}
% Reference to three sections.
\def\secrefs#1#2#3{sections \ref{#1}, \ref{#2} and \ref{#3}}
% Reference to an equation, lower-case.
\def\eqref#1{equation~\ref{#1}}
% Reference to an equation, upper case
\def\Eqref#1{Equation~\ref{#1}}
% A raw reference to an equation---avoid using if possible
\def\plaineqref#1{\ref{#1}}
% Reference to a chapter, lower-case.
\def\chapref#1{chapter~\ref{#1}}
% Reference to an equation, upper case.
\def\Chapref#1{Chapter~\ref{#1}}
% Reference to a range of chapters
\def\rangechapref#1#2{chapters\ref{#1}--\ref{#2}}
% Reference to an algorithm, lower-case.
\def\algref#1{algorithm~\ref{#1}}
% Reference to an algorithm, upper case.
\def\Algref#1{Algorithm~\ref{#1}}
\def\twoalgref#1#2{algorithms \ref{#1} and \ref{#2}}
\def\Twoalgref#1#2{Algorithms \ref{#1} and \ref{#2}}
% Reference to a part, lower case
\def\partref#1{part~\ref{#1}}
% Reference to a part, upper case
\def\Partref#1{Part~\ref{#1}}
\def\twopartref#1#2{parts \ref{#1} and \ref{#2}}

\def\ceil#1{\lceil #1 \rceil}
\def\floor#1{\lfloor #1 \rfloor}
\def\1{\bm{1}}
\newcommand{\train}{\mathcal{D}}
\newcommand{\valid}{\mathcal{D_{\mathrm{valid}}}}
\newcommand{\test}{\mathcal{D_{\mathrm{test}}}}

\def\eps{{\epsilon}}


% Random variables
\def\reta{{\textnormal{$\eta$}}}
\def\ra{{\textnormal{a}}}
\def\rb{{\textnormal{b}}}
\def\rc{{\textnormal{c}}}
\def\rd{{\textnormal{d}}}
\def\re{{\textnormal{e}}}
\def\rf{{\textnormal{f}}}
\def\rg{{\textnormal{g}}}
\def\rh{{\textnormal{h}}}
\def\ri{{\textnormal{i}}}
\def\rj{{\textnormal{j}}}
\def\rk{{\textnormal{k}}}
\def\rl{{\textnormal{l}}}
% rm is already a command, just don't name any random variables m
\def\rn{{\textnormal{n}}}
\def\ro{{\textnormal{o}}}
\def\rp{{\textnormal{p}}}
\def\rq{{\textnormal{q}}}
\def\rr{{\textnormal{r}}}
\def\rs{{\textnormal{s}}}
\def\rt{{\textnormal{t}}}
\def\ru{{\textnormal{u}}}
\def\rv{{\textnormal{v}}}
\def\rw{{\textnormal{w}}}
\def\rx{{\textnormal{x}}}
\def\ry{{\textnormal{y}}}
\def\rz{{\textnormal{z}}}

% Random vectors
\def\rvepsilon{{\mathbf{\epsilon}}}
\def\rvtheta{{\mathbf{\theta}}}
\def\rva{{\mathbf{a}}}
\def\rvb{{\mathbf{b}}}
\def\rvc{{\mathbf{c}}}
\def\rvd{{\mathbf{d}}}
\def\rve{{\mathbf{e}}}
\def\rvf{{\mathbf{f}}}
\def\rvg{{\mathbf{g}}}
\def\rvh{{\mathbf{h}}}
\def\rvu{{\mathbf{i}}}
\def\rvj{{\mathbf{j}}}
\def\rvk{{\mathbf{k}}}
\def\rvl{{\mathbf{l}}}
\def\rvm{{\mathbf{m}}}
\def\rvn{{\mathbf{n}}}
\def\rvo{{\mathbf{o}}}
\def\rvp{{\mathbf{p}}}
\def\rvq{{\mathbf{q}}}
\def\rvr{{\mathbf{r}}}
\def\rvs{{\mathbf{s}}}
\def\rvt{{\mathbf{t}}}
\def\rvu{{\mathbf{u}}}
\def\rvv{{\mathbf{v}}}
\def\rvw{{\mathbf{w}}}
\def\rvx{{\mathbf{x}}}
\def\rvy{{\mathbf{y}}}
\def\rvz{{\mathbf{z}}}

% Elements of random vectors
\def\erva{{\textnormal{a}}}
\def\ervb{{\textnormal{b}}}
\def\ervc{{\textnormal{c}}}
\def\ervd{{\textnormal{d}}}
\def\erve{{\textnormal{e}}}
\def\ervf{{\textnormal{f}}}
\def\ervg{{\textnormal{g}}}
\def\ervh{{\textnormal{h}}}
\def\ervi{{\textnormal{i}}}
\def\ervj{{\textnormal{j}}}
\def\ervk{{\textnormal{k}}}
\def\ervl{{\textnormal{l}}}
\def\ervm{{\textnormal{m}}}
\def\ervn{{\textnormal{n}}}
\def\ervo{{\textnormal{o}}}
\def\ervp{{\textnormal{p}}}
\def\ervq{{\textnormal{q}}}
\def\ervr{{\textnormal{r}}}
\def\ervs{{\textnormal{s}}}
\def\ervt{{\textnormal{t}}}
\def\ervu{{\textnormal{u}}}
\def\ervv{{\textnormal{v}}}
\def\ervw{{\textnormal{w}}}
\def\ervx{{\textnormal{x}}}
\def\ervy{{\textnormal{y}}}
\def\ervz{{\textnormal{z}}}

% Random matrices
\def\rmA{{\mathbf{A}}}
\def\rmB{{\mathbf{B}}}
\def\rmC{{\mathbf{C}}}
\def\rmD{{\mathbf{D}}}
\def\rmE{{\mathbf{E}}}
\def\rmF{{\mathbf{F}}}
\def\rmG{{\mathbf{G}}}
\def\rmH{{\mathbf{H}}}
\def\rmI{{\mathbf{I}}}
\def\rmJ{{\mathbf{J}}}
\def\rmK{{\mathbf{K}}}
\def\rmL{{\mathbf{L}}}
\def\rmM{{\mathbf{M}}}
\def\rmN{{\mathbf{N}}}
\def\rmO{{\mathbf{O}}}
\def\rmP{{\mathbf{P}}}
\def\rmQ{{\mathbf{Q}}}
\def\rmR{{\mathbf{R}}}
\def\rmS{{\mathbf{S}}}
\def\rmT{{\mathbf{T}}}
\def\rmU{{\mathbf{U}}}
\def\rmV{{\mathbf{V}}}
\def\rmW{{\mathbf{W}}}
\def\rmX{{\mathbf{X}}}
\def\rmY{{\mathbf{Y}}}
\def\rmZ{{\mathbf{Z}}}

% Elements of random matrices
\def\ermA{{\textnormal{A}}}
\def\ermB{{\textnormal{B}}}
\def\ermC{{\textnormal{C}}}
\def\ermD{{\textnormal{D}}}
\def\ermE{{\textnormal{E}}}
\def\ermF{{\textnormal{F}}}
\def\ermG{{\textnormal{G}}}
\def\ermH{{\textnormal{H}}}
\def\ermI{{\textnormal{I}}}
\def\ermJ{{\textnormal{J}}}
\def\ermK{{\textnormal{K}}}
\def\ermL{{\textnormal{L}}}
\def\ermM{{\textnormal{M}}}
\def\ermN{{\textnormal{N}}}
\def\ermO{{\textnormal{O}}}
\def\ermP{{\textnormal{P}}}
\def\ermQ{{\textnormal{Q}}}
\def\ermR{{\textnormal{R}}}
\def\ermS{{\textnormal{S}}}
\def\ermT{{\textnormal{T}}}
\def\ermU{{\textnormal{U}}}
\def\ermV{{\textnormal{V}}}
\def\ermW{{\textnormal{W}}}
\def\ermX{{\textnormal{X}}}
\def\ermY{{\textnormal{Y}}}
\def\ermZ{{\textnormal{Z}}}

% Vectors
\def\vzero{{\bm{0}}}
\def\vone{{\bm{1}}}
\def\vmu{{\bm{\mu}}}
\def\vtheta{{\bm{\theta}}}
\def\va{{\bm{a}}}
\def\vb{{\bm{b}}}
\def\vc{{\bm{c}}}
\def\vd{{\bm{d}}}
\def\ve{{\bm{e}}}
\def\vf{{\bm{f}}}
\def\vg{{\bm{g}}}
\def\vh{{\bm{h}}}
\def\vi{{\bm{i}}}
\def\vj{{\bm{j}}}
\def\vk{{\bm{k}}}
\def\vl{{\bm{l}}}
\def\vm{{\bm{m}}}
\def\vn{{\bm{n}}}
\def\vo{{\bm{o}}}
\def\vp{{\bm{p}}}
\def\vq{{\bm{q}}}
\def\vr{{\bm{r}}}
\def\vs{{\bm{s}}}
\def\vt{{\bm{t}}}
\def\vu{{\bm{u}}}
\def\vv{{\bm{v}}}
\def\vw{{\bm{w}}}
\def\vx{{\bm{x}}}
\def\vy{{\bm{y}}}
\def\vz{{\bm{z}}}

% Elements of vectors
\def\evalpha{{\alpha}}
\def\evbeta{{\beta}}
\def\evepsilon{{\epsilon}}
\def\evlambda{{\lambda}}
\def\evomega{{\omega}}
\def\evmu{{\mu}}
\def\evpsi{{\psi}}
\def\evsigma{{\sigma}}
\def\evtheta{{\theta}}
\def\eva{{a}}
\def\evb{{b}}
\def\evc{{c}}
\def\evd{{d}}
\def\eve{{e}}
\def\evf{{f}}
\def\evg{{g}}
\def\evh{{h}}
\def\evi{{i}}
\def\evj{{j}}
\def\evk{{k}}
\def\evl{{l}}
\def\evm{{m}}
\def\evn{{n}}
\def\evo{{o}}
\def\evp{{p}}
\def\evq{{q}}
\def\evr{{r}}
\def\evs{{s}}
\def\evt{{t}}
\def\evu{{u}}
\def\evv{{v}}
\def\evw{{w}}
\def\evx{{x}}
\def\evy{{y}}
\def\evz{{z}}

% Matrix
\def\mA{{\bm{A}}}
\def\mB{{\bm{B}}}
\def\mC{{\bm{C}}}
\def\mD{{\bm{D}}}
\def\mE{{\bm{E}}}
\def\mF{{\bm{F}}}
\def\mG{{\bm{G}}}
\def\mH{{\bm{H}}}
\def\mI{{\bm{I}}}
\def\mJ{{\bm{J}}}
\def\mK{{\bm{K}}}
\def\mL{{\bm{L}}}
\def\mM{{\bm{M}}}
\def\mN{{\bm{N}}}
\def\mO{{\bm{O}}}
\def\mP{{\bm{P}}}
\def\mQ{{\bm{Q}}}
\def\mR{{\bm{R}}}
\def\mS{{\bm{S}}}
\def\mT{{\bm{T}}}
\def\mU{{\bm{U}}}
\def\mV{{\bm{V}}}
\def\mW{{\bm{W}}}
\def\mX{{\bm{X}}}
\def\mY{{\bm{Y}}}
\def\mZ{{\bm{Z}}}
\def\mBeta{{\bm{\beta}}}
\def\mPhi{{\bm{\Phi}}}
\def\mLambda{{\bm{\Lambda}}}
\def\mSigma{{\bm{\Sigma}}}

% Tensor
\DeclareMathAlphabet{\mathsfit}{\encodingdefault}{\sfdefault}{m}{sl}
\SetMathAlphabet{\mathsfit}{bold}{\encodingdefault}{\sfdefault}{bx}{n}
\newcommand{\tens}[1]{\bm{\mathsfit{#1}}}
\def\tA{{\tens{A}}}
\def\tB{{\tens{B}}}
\def\tC{{\tens{C}}}
\def\tD{{\tens{D}}}
\def\tE{{\tens{E}}}
\def\tF{{\tens{F}}}
\def\tG{{\tens{G}}}
\def\tH{{\tens{H}}}
\def\tI{{\tens{I}}}
\def\tJ{{\tens{J}}}
\def\tK{{\tens{K}}}
\def\tL{{\tens{L}}}
\def\tM{{\tens{M}}}
\def\tN{{\tens{N}}}
\def\tO{{\tens{O}}}
\def\tP{{\tens{P}}}
\def\tQ{{\tens{Q}}}
\def\tR{{\tens{R}}}
\def\tS{{\tens{S}}}
\def\tT{{\tens{T}}}
\def\tU{{\tens{U}}}
\def\tV{{\tens{V}}}
\def\tW{{\tens{W}}}
\def\tX{{\tens{X}}}
\def\tY{{\tens{Y}}}
\def\tZ{{\tens{Z}}}


% Graph
\def\gA{{\mathcal{A}}}
\def\gB{{\mathcal{B}}}
\def\gC{{\mathcal{C}}}
\def\gD{{\mathcal{D}}}
\def\gE{{\mathcal{E}}}
\def\gF{{\mathcal{F}}}
\def\gG{{\mathcal{G}}}
\def\gH{{\mathcal{H}}}
\def\gI{{\mathcal{I}}}
\def\gJ{{\mathcal{J}}}
\def\gK{{\mathcal{K}}}
\def\gL{{\mathcal{L}}}
\def\gM{{\mathcal{M}}}
\def\gN{{\mathcal{N}}}
\def\gO{{\mathcal{O}}}
\def\gP{{\mathcal{P}}}
\def\gQ{{\mathcal{Q}}}
\def\gR{{\mathcal{R}}}
\def\gS{{\mathcal{S}}}
\def\gT{{\mathcal{T}}}
\def\gU{{\mathcal{U}}}
\def\gV{{\mathcal{V}}}
\def\gW{{\mathcal{W}}}
\def\gX{{\mathcal{X}}}
\def\gY{{\mathcal{Y}}}
\def\gZ{{\mathcal{Z}}}

% Sets
\def\sA{{\mathbb{A}}}
\def\sB{{\mathbb{B}}}
\def\sC{{\mathbb{C}}}
\def\sD{{\mathbb{D}}}
% Don't use a set called E, because this would be the same as our symbol
% for expectation.
\def\sF{{\mathbb{F}}}
\def\sG{{\mathbb{G}}}
\def\sH{{\mathbb{H}}}
\def\sI{{\mathbb{I}}}
\def\sJ{{\mathbb{J}}}
\def\sK{{\mathbb{K}}}
\def\sL{{\mathbb{L}}}
\def\sM{{\mathbb{M}}}
\def\sN{{\mathbb{N}}}
\def\sO{{\mathbb{O}}}
\def\sP{{\mathbb{P}}}
\def\sQ{{\mathbb{Q}}}
\def\sR{{\mathbb{R}}}
\def\sS{{\mathbb{S}}}
\def\sT{{\mathbb{T}}}
\def\sU{{\mathbb{U}}}
\def\sV{{\mathbb{V}}}
\def\sW{{\mathbb{W}}}
\def\sX{{\mathbb{X}}}
\def\sY{{\mathbb{Y}}}
\def\sZ{{\mathbb{Z}}}

% Entries of a matrix
\def\emLambda{{\Lambda}}
\def\emA{{A}}
\def\emB{{B}}
\def\emC{{C}}
\def\emD{{D}}
\def\emE{{E}}
\def\emF{{F}}
\def\emG{{G}}
\def\emH{{H}}
\def\emI{{I}}
\def\emJ{{J}}
\def\emK{{K}}
\def\emL{{L}}
\def\emM{{M}}
\def\emN{{N}}
\def\emO{{O}}
\def\emP{{P}}
\def\emQ{{Q}}
\def\emR{{R}}
\def\emS{{S}}
\def\emT{{T}}
\def\emU{{U}}
\def\emV{{V}}
\def\emW{{W}}
\def\emX{{X}}
\def\emY{{Y}}
\def\emZ{{Z}}
\def\emSigma{{\Sigma}}

% entries of a tensor
% Same font as tensor, without \bm wrapper
\newcommand{\etens}[1]{\mathsfit{#1}}
\def\etLambda{{\etens{\Lambda}}}
\def\etA{{\etens{A}}}
\def\etB{{\etens{B}}}
\def\etC{{\etens{C}}}
\def\etD{{\etens{D}}}
\def\etE{{\etens{E}}}
\def\etF{{\etens{F}}}
\def\etG{{\etens{G}}}
\def\etH{{\etens{H}}}
\def\etI{{\etens{I}}}
\def\etJ{{\etens{J}}}
\def\etK{{\etens{K}}}
\def\etL{{\etens{L}}}
\def\etM{{\etens{M}}}
\def\etN{{\etens{N}}}
\def\etO{{\etens{O}}}
\def\etP{{\etens{P}}}
\def\etQ{{\etens{Q}}}
\def\etR{{\etens{R}}}
\def\etS{{\etens{S}}}
\def\etT{{\etens{T}}}
\def\etU{{\etens{U}}}
\def\etV{{\etens{V}}}
\def\etW{{\etens{W}}}
\def\etX{{\etens{X}}}
\def\etY{{\etens{Y}}}
\def\etZ{{\etens{Z}}}

% The true underlying data generating distribution
\newcommand{\pdata}{p_{\rm{data}}}
% The empirical distribution defined by the training set
\newcommand{\ptrain}{\hat{p}_{\rm{data}}}
\newcommand{\Ptrain}{\hat{P}_{\rm{data}}}
% The model distribution
\newcommand{\pmodel}{p_{\rm{model}}}
\newcommand{\Pmodel}{P_{\rm{model}}}
\newcommand{\ptildemodel}{\tilde{p}_{\rm{model}}}
% Stochastic autoencoder distributions
\newcommand{\pencode}{p_{\rm{encoder}}}
\newcommand{\pdecode}{p_{\rm{decoder}}}
\newcommand{\precons}{p_{\rm{reconstruct}}}

\newcommand{\laplace}{\mathrm{Laplace}} % Laplace distribution

\newcommand{\E}{\mathbb{E}}
\newcommand{\Ls}{\mathcal{L}}
\newcommand{\R}{\mathbb{R}}
\newcommand{\emp}{\tilde{p}}
\newcommand{\lr}{\alpha}
\newcommand{\reg}{\lambda}
\newcommand{\rect}{\mathrm{rectifier}}
\newcommand{\softmax}{\mathrm{softmax}}
\newcommand{\sigmoid}{\sigma}
\newcommand{\softplus}{\zeta}
\newcommand{\KL}{D_{\mathrm{KL}}}
\newcommand{\Var}{\mathrm{Var}}
\newcommand{\standarderror}{\mathrm{SE}}
\newcommand{\Cov}{\mathrm{Cov}}
% Wolfram Mathworld says $L^2$ is for function spaces and $\ell^2$ is for vectors
% But then they seem to use $L^2$ for vectors throughout the site, and so does
% wikipedia.
\newcommand{\normlzero}{L^0}
\newcommand{\normlone}{L^1}
\newcommand{\normltwo}{L^2}
\newcommand{\normlp}{L^p}
\newcommand{\normmax}{L^\infty}

\newcommand{\parents}{Pa} % See usage in notation.tex. Chosen to match Daphne's book.

\DeclareMathOperator*{\argmax}{arg\,max}
\DeclareMathOperator*{\argmin}{arg\,min}

\DeclareMathOperator{\sign}{sign}
\DeclareMathOperator{\Tr}{Tr}
\let\ab\allowbreak


==> tables/flow.tex <==
\begin{table}[]
% \begin{wraptable}{r}{{0.5\textwidth}}
% \vspace{-\baselineskip}
\centering
\caption{Experiment results on Flow.}
\label{table:flow}
\renewcommand{\arraystretch}{1.2}
{
\begin{adjustbox}{width=0.9\textwidth}
\begin{tabular}{lcccccccc}
\hlineB{3}
\multicolumn{1}{c|}{\multirow{2}{*}{Models}} & \multicolumn{8}{c}{Flow}                                                                                                                                                                             \\ \cline{2-9} 
\multicolumn{1}{c|}{}                        & MIC $\mathbf{\uparrow}$                   & TIC $\mathbf{\uparrow}$                   & PosMIC   $\mathbf{\uparrow}$              & PosTIC   $\mathbf{\uparrow}$              & NegMIC   $\mathbf{\downarrow}$              & NegTIC $\mathbf{\downarrow}$               & $F_1^{MIC}$  $\mathbf{\uparrow}$               & $F_1^{TIC}$  $\mathbf{\uparrow}$               \\ \hline
\multicolumn{9}{c}{\textit{Fully supervised learning methods (all labels are used)}}                                                                                                                                                                \\ \hline
\multicolumn{1}{l|}{CausalVAE \cite{DBLP:conf/cvpr/YangLCSHW21}}               & 72.1 $\pm$1.3          & 56.4 $\pm$1.6          & 45.1 $\pm$4.8          & 36.7 $\pm$4.2          & 43.3 $\pm$5.1          & 33.7 $\pm$3.2         & 50.2 $\pm$4.4          & 47.3 $\pm$3.7          \\
\multicolumn{1}{l|}{ConditionVAE \cite{bib:conditionvae}}            & \textbf{75.5 $\pm$2.3} & \textbf{56.5 $\pm$1.8} & 28.6 $\pm$3.2 & 21.3 $\pm$3.1          & 27.2 $\pm$2.8          & 20.6 $\pm$2.7         & 41.1 $\pm$5.1          & 33.6 $\pm$4.0          \\ \hline
\multicolumn{9}{c}{\textit{Unsupervised learning methods  (no labels is used)}}                                                                                                                                                                     \\ \hline
\multicolumn{1}{l|}{CausalVAE(unsup) \cite{DBLP:conf/cvpr/YangLCSHW21}}        & 20.5 $\pm$4.7          & 11.8 $\pm$2.6          & 22.8 $\pm$2.7          & 12.5 $\pm$1.4          & 21.5 $\pm$2.4          & 12.0 $\pm$1.9         & 35.3 $\pm$5.6          & 21.9 $\pm$4.7          \\
\multicolumn{1}{l|}{betaVAE}                 & 23.6 $\pm$3.2          & 12.5 $\pm$0.6          & 23.6 $\pm$3.6          & 12.5 $\pm$1.9          & 22.1 $\pm$2.5          & 11.4 $\pm$1.9         & 36.2 $\pm$4.9          & 21.9 $\pm$4.2          \\
\multicolumn{1}{l|}{LadderVAE \cite{bib:laddervae}}               & 34.3 $\pm$4.3          & 24.4 $\pm$1.5          & 16.2 $\pm$1.8          & 10.5 $\pm$1.0          & \textbf{13.3 $\pm$1.2} & \textbf{6.9 $\pm$0.6} & 27.3 $\pm$ 3.2         & 18.9 $\pm$2.8          \\ \hline
\multicolumn{9}{c}{\textit{Reduced supervision method (no label is used; Supervision source is image pairing)}}                                                                                                                                     \\ \hline
% \multicolumn{1}{l|}{LCM \cite{bib:weakly-causal}}              & 55.1 $\pm$5.7          & 45.3 $\pm$4.1          & 47.1 $\pm$3.9 & 39.3 $\pm$4.7 & 37.8 $\pm$5.2          & 29.9 $\pm$4.2         & 52.9 $\pm$4.5 & 50.3 $\pm$3.7 \\ 
\multicolumn{1}{l|}{Our method}              & 65.5 $\pm$6.6          & 56.7 $\pm$4.9          & \textbf{50.7 $\pm$4.7} & \textbf{41.3 $\pm$4.2} & 36.8 $\pm$3.8 & 27.2 $\pm$3.0         & \textbf{56.3 $\pm$5.9} & \textbf{52.7 $\pm$4.9} \\ \hlineB{3}
\end{tabular}
\end{adjustbox}
}
% \vspace{-\baselineskip}
% \end{wraptable}
\end{table}

==> tables/harmonyMIC.tex <==
\begin{table}[]
\tiny
\centering
\caption{Causal representation learning evaluated by $F_1^{MIC}$ and $F_1^{TIC}$ tested on Pendulum and Flow datasets}
\label{table:harmonymic}
\renewcommand{\arraystretch}{1.3}
{
\begin{adjustbox}{width=0.8\textwidth}
\begin{tabular}{ccccc}
\hlineB{2}
\multicolumn{1}{c|}{\multirow{2}{*}{Models}}  & \multicolumn{2}{c|}{Pendulum}                                        & \multicolumn{2}{c}{Flow}                                        \\ \cline{2-5} 
\multicolumn{1}{c|}{}                         & \multicolumn{1}{l}{$F_1^{MIC}$ $\uparrow$} & \multicolumn{1}{l|}{$F_1^{TIC}$ $\uparrow$ }     & \multicolumn{1}{l}{$F_1^{MIC}$ $\uparrow$} & \multicolumn{1}{l}{$F_1^{TIC}$ $\uparrow$} \\ \hline
\multicolumn{5}{c}{\textit{Fully supervised learning methods (all labels are used)}}                                                                                                            \\ \hline
\multicolumn{1}{c|}{CausalVAE \cite{DBLP:conf/cvpr/YangLCSHW21}}                & 53.20                          & \multicolumn{1}{c|}{51.39}          & 50.24                          & 47.25                          \\
\multicolumn{1}{c|}{ConditionVAE \cite{bib:conditionvae}}             & 46.85                          & \multicolumn{1}{c|}{40.46}          & 41.07                          & 33.59                          \\ \hline
\multicolumn{5}{c}{\textit{Unsupervised learning methods (no label is used)}}                                                                                                                   \\ \hline
\multicolumn{1}{c|}{CausalVAE(unsup) \cite{DBLP:conf/cvpr/YangLCSHW21}} & 32.35                          & \multicolumn{1}{c|}{20.73}          & 35.34                          & 21.89                          \\
\multicolumn{1}{c|}{betaVAE \cite{DBLP:conf/iclr/HigginsMPBGBML17}}                  & 33.18                          & \multicolumn{1}{c|}{22.17}          & 36.23                          & 21.91                          \\
\multicolumn{1}{c|}{LadderVAE \cite{bib:laddervae}}                & 25.82                          & \multicolumn{1}{c|}{15.73}          & 27.30                          & 18.87                          \\ \hline
\multicolumn{5}{c}{\textit{Reduced learning method (a pair of inputs are used but no label is used)}}                                                                                           \\ \hline
\multicolumn{1}{c|}{Our method}               & \textbf{56.81}                 & \multicolumn{1}{c|}{\textbf{53.55}} & \textbf{56.26}                 & \textbf{52.70}                 \\ \hlineB{2}
\end{tabular}
\end{adjustbox}
}
\end{table}



==> tables/pendulum.tex <==
\begin{table}[]
% \begin{wraptable}{l}{{0.5\textwidth}}
% \vspace{-\baselineskip}
\centering
\caption{Experiment results on Pendulum.  }
\label{table:pendulum}
\renewcommand{\arraystretch}{1.2}
{
\begin{adjustbox}{width=0.9\textwidth}
\begin{tabular}{lcccccccc}
\hline
\multicolumn{1}{c|}{\multirow{2}{*}{Models}} & \multicolumn{8}{c}{Pendulum}                                                                                                                                                                         \\ \cline{2-9} 
\multicolumn{1}{c|}{}                        & MIC $\mathbf{\uparrow}$                    & TIC $\mathbf{\uparrow}$                    & PosMIC $\mathbf{\uparrow}$                & PosTIC $\mathbf{\uparrow}$                & NegMIC $\mathbf{\downarrow}$             & NegTIC $\mathbf{\downarrow}$              & $F_1^{MIC}$ $\mathbf{\uparrow}$                 & $F_1^{TIC}$ $\mathbf{\uparrow}$                \\ \hline
\multicolumn{9}{c}{\textit{Fully supervised learning methods (all labels are used)}}                                                                                                                                                                \\ \hline
\multicolumn{1}{l|}{CausalVAE \cite{DBLP:conf/cvpr/YangLCSHW21}}               & \textbf{95.1 $\pm$2.4} & \textbf{81.6 $\pm$1.9} & 53.0 $\pm$4.5          & 43.4 $\pm$3.7          & 46.6 $\pm$3.9          & 37.0 $\pm$4.2         & 53.2 $\pm$3.6          & 51.4 $\pm$3.2          \\
\multicolumn{1}{l|}{ConditionVAE \cite{bib:conditionvae}}            & 93.8 $\pm$3.3          & 80.5 $\pm$1.4          & 36.5 $\pm$3.0          & 27.8 $\pm$3.2          & 34.6 $\pm$4.2          & 25.7 $\pm$3.6         & 46.9 $\pm$4.7          & 40.5 $\pm$3.5          \\ \hline
\multicolumn{9}{c}{\textit{Unsupervised learning methods (no label is used)}}                                                                                                                                                                       \\ \hline
\multicolumn{1}{l|}{CausalVAE(unsup) \cite{DBLP:conf/cvpr/YangLCSHW21}}        & 21.2 $\pm$1.4          & 12.0 $\pm$1.0          & 20.5 $\pm$2.6          & 11.8 $\pm$2.7          & 23.3 $\pm$3.2          & 14.7 $\pm$1.9         & 32.4 $\pm$3.4          & 20.7 $\pm$3.1          \\
\multicolumn{1}{l|}{$\beta$-VAE \cite{DBLP:conf/iclr/HigginsMPBGBML17}}             & 22.6 $\pm$4.6          & 12.5 $\pm$2.2          & 21.2 $\pm$2.7          & 12.7 $\pm$2.9          & 23.7 $\pm$3.1          & 12.6 $\pm$1.9         & 33.2 $\pm$3.3          & 22.2 $\pm$2.7          \\
\multicolumn{1}{l|}{LadderVAE \cite{bib:laddervae}}               & 22.4 $\pm$3.1          & 12.8 $\pm$1.2          & 15.2 $\pm$1.9          & 8.6 $\pm$1.0           & \textbf{14.2 $\pm$1.7} & \textbf{7.9 $\pm$0.9} & 25.8 $\pm$3.0          & 15.7 $\pm$2.8          \\ \hline
\multicolumn{9}{c}{\textit{Reduced supervision method (no label is used; Supervision source is image pairing)}}                                                                                                                                     \\ \hline
% \multicolumn{1}{l|}{LCM \cite{bib:weakly-causal} }              & 80.1 $\pm$6.7          & 71.3 $\pm$6.1          & 50.1 $\pm$4.9 & 40.3 $\pm$4.4 & 43.2 $\pm$4.2          & 34.9 $\pm$3.9         & 53.4 $\pm$5.5 & 50.1 $\pm$4.7 \\ 
\multicolumn{1}{l|}{Our method}              & 86.6 $\pm$7.9          & 74.5 $\pm$5.1          & \textbf{54.1 $\pm$4.5} & \textbf{44.0 $\pm$4.2} & 40.2 $\pm$3.9          & 31.6 $\pm$3.2         & \textbf{56.8 $\pm$5.2} & \textbf{53.6 $\pm$4.3} \\ \hline
\end{tabular}

\end{adjustbox}
}
% \vspace{-\baselineskip}
% \end{wraptable}
% \leavevmode
\end{table}
